Orthogonal Projection Loss

Deep neural networks have achieved remarkable performance on a range of classification tasks, with softmax cross-entropy (CE) loss emerging as the de-facto objective function. The CE loss encourages features of a class to have a higher projection score on the true class-vector compared to the negative classes. However, this is a relative constraint and does not explicitly force different class features to be well-separated. Motivated by the observation that ground-truth class representations in CE loss are orthogonal (one-hot encoded vectors), we develop a novel loss function termed `Orthogonal Projection Loss' (OPL) which imposes orthogonality in the feature space. OPL augments the properties of CE loss and directly enforces inter-class separation alongside intra-class clustering in the feature space through orthogonality constraints on the mini-batch level. As compared to other alternatives of CE, OPL offers unique advantages e.g., no additional learnable parameters, does not require careful negative mining and is not sensitive to the batch size. Given the plug-and-play nature of OPL, we evaluate it on a diverse range of tasks including image recognition (CIFAR-100), large-scale classification (ImageNet), domain generalization (PACS) and few-shot learning (miniImageNet, CIFAR-FS, tiered-ImageNet and Meta-dataset) and demonstrate its effectiveness across the board. Furthermore, OPL offers better robustness against practical nuisances such as adversarial attacks and label noise. Code is available at: https://github.com/kahnchana/opl.

==> figures/ablation_lambda.tex <==
\begin{figure}[]
    \centering
    \includegraphics[width=\linewidth]{figures/plots/ablation/lambda.png}
    \vspace{-2mm}
	\caption{\textbf{Performance sensitivity to lambda:} Minor variations of lambda parameter in OPL continues to provide improvements over the CE baseline. Experiments conducted on CIFAR-100 dataset with a ResNet-56 backbone.}
	\label{fig:ablation_lambda}
\end{figure}






% \begin{table}[]
% \centering
% \begin{tabular}{c|c|c|c}
% \hline
% hyper-parameter      & $\gamma$=2             & $\gamma$=1       & $\gamma$=0.5   \\ \hline \hline
% $\lambda$ = 0^\dagger        & 72.40                  & 72.40            & 72.40 \\ \hline
% $\lambda$ = 0.05             & 72.77                  & 73.32            & 73.07 \\ \hline
% $\lambda$ = 0.1              & 72.39                  & \textbf{73.56}   & 73.17 \\ \hline
% $\lambda$ = 0.5              & 72.18                  & 72.24            & 72.40 \\ \hline
% $\lambda$ = 1.0              & 71.23                  & 72.30            & 73.34 \\ \hline
% $\lambda$ = 2.0              & 71.10                  & 71.43            & 72.10 \\ \hline
% \end{tabular}
% \caption{\textbf{Sensitivity Analysis:} We report the variation of top-1 accuracy (\%) on CIFAR-100 test set with various pairs of $\lambda$ and $\gamma$ hyper-parameters ($^{\dagger}$ indicates no OPL case).}
% \label{table:search_table}
% \end{table}



==> figures/baseline_cifar100.tex <==
\begin{table}[]
	\small
	\begin{center}
    \begin{tabular}{|l|c|c|c|c|}
    \toprule[0.4mm]
    \rowcolor{mygray} \multirow{2}{*}{Method} 
              & \multicolumn{2}{c|}{CIFAR-10} & \multicolumn{2}{c|}{CIFAR-100} \\ \cline{2-5}
              & ResNet50      & ResNet100     & ResNet50      & ResNet101      \\ \hline
    Baseline  & ??.??\%       & ??.??\%       & 77.39\%       & 77.78\%        \\ \hline
    OPL       & ??.??\%       & ??.??\%       & \textbf{78.70\%} & \textbf{79.03\%} \\ \bottomrule[0.4mm]
    \end{tabular}
	\end{center}
	\caption{\textbf{Results on CIFAR-10 \& CIFAR-100:} We explore the effects of applying OPL on common RESNET architectures. OPL improves performance over the baseline for all cases.}
	\label{table:baseline_cifar100}
\end{table}

==> figures/class_separation_importance.tex <==
\begin{figure}[t]
	\begin{center}
		\includegraphics[width=0.9\linewidth]{figures/plots/class_separation_importance.png}
	\end{center}
	\caption{As shown in \cite{unravelling_meta}, the inter-class to intra-class variation ratio significantly affects the performance of a feature embedding when used for few-shot learning tasks. \hl{Make this more general: relate to generalizable feature representations. Change this plot: this is from another paper.}}
	\label{fig:class_separation_importance}
\end{figure}


==> figures/comparison_metadataset_imnet.tex <==
\begin{table}[]
\begin{center}
	\small
	\begin{tabular}{l|c|c|c}
	\toprule[0.4mm]
	\rowcolor{mygray} 
	Dataset       & RFS \cite{rfs_paper} & MB \cite{meta_baseline_paper} & Ours \\ \midrule
	Imagenet      &     & 59.2 &      \\ \hline
	Omniglot      &     & 69.1 &      \\ \hline
	Aircraft      &     & 54.1 &      \\ \hline
	Birds         &     & 77.3 &      \\ \hline
	Textures      &     & 76.0 &      \\ \hline
	Quick Draw    &     & 57.3 &      \\ \hline
	Fungi         &     & 45.4 &      \\ \hline
	VGG Flower    &     & 89.6 &      \\ \hline
	Traffic Signs &     & 66.2 &      \\ \hline
	MSCOCO        &     & 55.7 &      \\ \bottomrule[0.4mm]
\end{tabular}
\caption{\textbf{Results on Meta-Dataset}: We obtain our results by performing the base supervised training in \cite{meta_baseline_paper} jointly with OPL loss alongside CE. Reported results are for models trained only on the ImageNet training split of Meta-Dataset.}
\end{center}
\label{table:comparison_metadataset_imnet}
\end{table}


==> figures/lda_analysis_cifar100.tex <==
\begin{figure}[t]
	\begin{center}
		\includegraphics[width=0.9\linewidth]{figures/plots/lda_cifar100_ce.png}
		\includegraphics[width=0.9\linewidth]{figures/plots/lda_cifar100_opl.png}
	\end{center}
	\caption{Comparison of feature space for models trained with and without OPL. The intended inter-class separation and intra-class clustering can be observed. The features of a ResNet50 model have been projected to 2 dimensions using LDA and the first two components of LDA are plotted against each other. }
	\label{fig:lda_analysis_cifar100}
\end{figure}


